Simple, Distributed, and Accelerated Probabilistic Programming

We describe a simple, low-level approach for embedding probabilistic programming in a deep learning ecosystem. In particular, we distill probabilistic programming down to a single abstraction---the random variable. Our lightweight implementation in TensorFlow enables numerous applications: a model-parallel variational auto-encoder (VAE) with 2nd-generation tensor processing units (TPUv2s); a data-parallel autoregressive model (Image Transformer) with TPUv2s; and multi-GPU No-U-Turn Sampler (NUTS). For both a state-of-the-art VAE on 64x64 ImageNet and Image Transformer on 256x256 CelebA-HQ, our approach achieves an optimal linear speedup from 1 to 256 TPUv2 chips. With NUTS, we see a 100x speedup on GPUs over Stan and 37x over PyMC3.

==> tikz/distributed_flow_dots.tex <==
\begin{tikzpicture}

  % Nodes
  \node[obs, minimum size=0.4cm] (x) {};
  
  \node[below=of x, yshift=0.4cm, minimum size=0.4cm] (h0c) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=-2.0cm] (h00) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=-0.75cm] (h01) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=0.75cm] (h02) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=2.0cm] (h03) {};
  
  \node[below=of h0c, yshift=0.4cm, minimum size=0.4cm] (h1c) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=-2.0cm] (h10) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=-0.75cm] (h11) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=0.75cm] (h12) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=2.0cm] (h13) {};
  
  \node[below=of h1c, yshift=0.5cm, minimum size=0.4cm] (dots) {$\cdots$};
  
  \node[below=of dots, yshift=0.4cm, minimum size=0.4cm] (h2c) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=-2.0cm] (h20) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=-0.7cm] (h21) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=0.7cm] (h22) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=2.0cm] (h23) {};
  
  \node[below=of h2c, yshift=0.4cm, minimum size=0.4cm] (h3c) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=-2.0cm] (h30) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=-0.7cm] (h31) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=0.7cm] (h32) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=2.0cm] (h33) {};
  
  \node[obs, minimum size=0.4cm, below=of h3c, yshift=0.4cm] (y) {};

  % Plates
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate0} {
    (h00)(h10)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate1} {
    (h01)(h11)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate2} {
    (h02)(h12)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate3} {
    (h03)(h13)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate20} {
    (h20)(h30)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate21} {
    (h21)(h31)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate22} {
    (h22)(h32)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate23} {
    (h23)(h33)
  } {};
  \plate[inner sep=0.2cm, yshift=0.2cm, fill=SkyBlue, text opacity=1] {plate9} {
    (y)
  } {};

  % Edges
  \edge{x}{h00}
  \edge{x}{h01}
  \edge{x}{h02}
  \edge{x}{h03}
  
  \edge{h00}{h10};
  \edge{h01}{h10};
%   \edge{h02}{h10};
%   \edge{h03}{h10};
  \edge{h00}{h11};
  \edge{h01}{h11};
  \edge{h02}{h11};
%   \edge{h03}{h11};
%   \edge{h00}{h12};
  \edge{h01}{h12};
  \edge{h02}{h12};
  \edge{h03}{h12};
%   \edge{h00}{h13};
%   \edge{h01}{h13};
  \edge{h02}{h13};
  \edge{h03}{h13};
  
  \edge[thick]{h10}{dots};
  \edge[thick]{h11}{dots};
  \edge[thick]{h12}{dots};
  \edge[thick]{h13}{dots};
  
  \edge[thick]{dots}{h20};
  \edge[thick]{dots}{h21};
  \edge[thick]{dots}{h22};
  \edge[thick]{dots}{h23};
  
  \edge{h20}{h30};
  \edge{h21}{h30};
%   \edge{h22}{h30};
%   \edge{h23}{h30};
  \edge{h20}{h31};
  \edge{h21}{h31};
  \edge{h22}{h31};
%   \edge{h23}{h31};
%   \edge{h20}{h32};
  \edge{h21}{h32};
  \edge{h22}{h32};
  \edge{h23}{h32};
%   \edge{h20}{h33};
%   \edge{h21}{h33};
  \edge{h22}{h33};
  \edge{h23}{h33};
  
  \edge{h30}{y};
  \edge{h31}{y};
  \edge{h32}{y};
  \edge{h33}{y};

  % Nodes: I redrew them here to preserve node colors
  \node[obs, minimum size=0.4cm] (x) {};
  
  \node[below=of x, yshift=0.4cm, minimum size=0.4cm] (h0c) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=-2.0cm] (h00) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=-0.75cm] (h01) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=0.75cm] (h02) {};
  \node[obs, minimum size=0.4cm, below=of x, yshift=0.4cm, xshift=2.0cm] (h03) {};
  
  \node[below=of h0c, yshift=0.4cm, minimum size=0.4cm] (h1c) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=-2.0cm] (h10) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=-0.75cm] (h11) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=0.75cm] (h12) {};
  \node[obs, minimum size=0.4cm, below=of h0c, yshift=0.4cm, xshift=2.0cm] (h13) {};
  
  \node[below=of h1c, yshift=0.5cm, minimum size=0.4cm] (dots) {$\cdots$};
  
  \node[below=of dots, yshift=0.4cm, minimum size=0.4cm] (h2c) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=-2.0cm] (h20) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=-0.75cm] (h21) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=0.75cm] (h22) {};
  \node[obs, minimum size=0.4cm, below=of dots, yshift=0.4cm, xshift=2.0cm] (h23) {};
  
  \node[below=of h2c, yshift=0.4cm, minimum size=0.4cm] (h3c) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=-2.0cm] (h30) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=-0.75cm] (h31) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=0.75cm] (h32) {};
  \node[obs, minimum size=0.4cm, below=of h2c, yshift=0.4cm, xshift=2.0cm] (h33) {};
  
  \node[obs, minimum size=0.4cm, below=of h3c, yshift=0.4cm] (y) {};

\end{tikzpicture}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

